Optimal and Robust Fault Tolerant Control of Wind Turbines Working under Sensor, Actuator, and System Faults

Motivated by the increasing concerns over environmental challenges such as global warming and the exhaustion of fossil-fuel reserves, the renewable energy industry has become the most demanded electrical energy production source worldwide. In this context, wind energy conversion systems (WECSs) are the most dominant and fastest-growing alternative energy production technologies, playing an increasingly vital role in renewable power generation. To tackle the pitch control problem of WECSs, this thesis proposes an optimal fault-tolerant fractional-order pitch control strategy for pitch angle regulation of WT blades subjected to sensor, actuator, and system faults. To showcast the effects of faults, changes in the system parameters are considered as a result of sensor, actuator and system faults with various levels of severity.} Furthermore, taking advantage of the favourable merits of higher-order SMCs and fractional calculus, this thesis develops a fault-tolerant fractional-calculus-based higher-order sliding mode controller for optimum rotor speed tracking and power production maximization of WECSs. \textcolor{black}{The partial loss of the generator output torque is considered as an actuator failure, leading to loss of partial actuation power. Moreover, active fault-tolerant fractional-order higher-order SMC strategies are developed for rotor current regulation and speed trajectory tracking of doubly-fed induction generator (DFIG) -driven WECSs subjected to model uncertainties and rotor current sensor faults. The developed controllers are augmented with two state observers, an algebraic state estimator and a sliding mode observer, to estimate the rotor current dynamics during sensors' faults.

==> Chapters/Chapter0.tex <==
\chapter{List of Publications} % Main chapter title

\label{Chapter0}

\section{Published Publications}
\begin{enumerate}
  \item \href{https://www.sciencedirect.com/science/article/pii/S1364032122006232}{\textbf{Y. Mousavi}, G. Bevan, I. B. Kucukdemiral, A. Fekih, "Sliding mode control of wind energy conversion systems: trends and applications," \textit{Renewable and Sustainable Energy Reviews}, 167, 2022.}
  \item \textbf{Y. Mousavi}, G. Bevan, I. B. Kucukdemiral, A. Fekih, "Active fault-tolerant fractional-order terminal sliding mode control for DFIG-based wind turbines subjected to sensor faults," \textit{2022 IEEE IAS Global Conference on Emerging Technologies (GlobConET), May 2022}.
  \item \href{https://www.sciencedirect.com/science/article/pii/S0019057821005383}{\textbf{Y. Mousavi}, G. Bevan, I. B. Kucukdemiral, "Fault-tolerant optimal pitch control of wind turbines using dynamic weighted parallel firefly algorithm," \textit{ISA Transactions}, 2021.}
  \item \href{https://www.mdpi.com/1996-1073/14/18/5887}{\textbf{Y. Mousavi}, G. Bevan, I. B. Kucukdemiral, A. Fekih, "Maximum power extraction from wind turbines using a fault-tolerant fractional-order nonsingular terminal sliding mode controller," \textit{Energies}, 14(18), 2021.}
\end{enumerate} 

\section{Ready for Submission}
\begin{enumerate}
  \item \textbf{Y. Mousavi}, G. Bevan, I. B. Kucukdemiral, A. Fekih, "Fault-tolerant observer-based Higher-order Sliding Mode Control of DFIG-based Wind Turbines with Sensor Faults," \textit{to be submitted to IEEE Transactions on Industry Applications}.
\end{enumerate}

